Identifying Health Risks from Family History: A Survey of Natural Language Processing Techniques

Electronic health records include information on patients' status and medical history, which could cover the history of diseases and disorders that could be hereditary. One important use of family history information is in precision health, where the goal is to keep the population healthy with preventative measures. Natural Language Processing (NLP) and machine learning techniques can assist with identifying information that could assist health professionals in identifying health risks before a condition is developed in their later years, saving lives and reducing healthcare costs. We survey the literature on the techniques from the NLP field that have been developed to utilise digital health records to identify risks of familial diseases. We highlight that rule-based methods are heavily investigated and are still actively used for family history extraction. Still, more recent efforts have been put into building neural models based on large-scale pre-trained language models. In addition to the areas where NLP has successfully been utilised, we also identify the areas where more research is needed to unlock the value of patients' records regarding data collection, task formulation and downstream applications.

==> csur-archived/body.tex <==
\section{Introduction}

\paragraph{what is family history and why it is useful}
The value of family history information has long been recognized.

Family history, genetic susceptibility, shared environmental and behavioral factors.

Cardiovascular diseases, type 2 diabetes, many cancers.

Different from genetic susceptibility that can be obtained via genetic profiling, family history information captures the complex interactions between genetic, environmental, and behavioral factors.



\subparagraph{A motivating example}
\begin{itemize}
    \item Pancreatic cancer is the fourth leading cause of cancer death in the United States, while an estimated 466,003 people died from it worldwide in 2020.~\footnote{\url{https://www.cancer.net/cancer-types/pancreatic-cancer/statistics}}
    \item Due to its few sign and symptoms until in well-advanced cancer stages, pancreatic cancer is referred to as silent killer: around 73\% patients die within the first year of their diagnosis~\citep{mehrabi-mayo-2015-family-history}.
    \item Several risk factors such as family history, pancreatic cysts, obesity, smoking, and alcohol intake have been found:
    \begin{itemize}
        \item It is estimated that 10\% of pancreatic cancers have a familial basis.
        \item Risk is increased 7-9 fold if one first-degree relative (parents, siblings or children) has pancreatic cancer.
    \end{itemize}
    \item Other examples include the risk assessment of hypertrophic cardiomyopathy~\cite{shen-mayo-2021-jmir-n2c2-2019-fh}.
\end{itemize}

We are interested in identifying health risks from patient-centred data, including medical history, family history and social history (social determinants of health).

\begin{itemize}
    \item Social determinants of health (SDOH) are the conditions in which people live that affect quality-of-life and health outcomes.\footnote{\url{https://health.gov/healthypeople/priority-areas/social-determinants-health}}
\end{itemize}

\citet{milne-auckland-2009-family-hisory} study the associations between family history of four psychiatric disorders---depression, anxiety, alcohol dependence and drug dependence---and clinical features of these disorders in probands (the first diagnosed family member). They suggest that family history is useful for determining patients' clinical prognosis and for selecting cases for genetic studies.

Family history can be used to estimate the risk of a patient developing certain diseases such as breast cancer, colorectal cancer, ovarian cancer, osteoporosis, cardiovascular disease, psychiatric disorders, and diabetes~\citep{polubriaginof-columbia-2015-amia-family-history}.
It can also signal the need for further genetic counseling or preventative health screening~\citep{bill-minnesota-2014-amia-family-history}.
For example, \citet{permuth-egan-2009-familial-cancer} find that individuals with a family history of pancreatic cancer have nearly a two-fold increased risk for developing pancreatic cancer to those without such a history.
They suggest that families with two or more pancreatic cancer cases may benefit from comprehensive risk assessment using detailed family history data, and that those at highest risk may be referred to screening programs.

In addition to risk assessment, \citet{claassen-vumc-2010-bmc-family-history} point out that family history information can be used to personalize health messages, which motivate at-risk individuals to adopt and maintain healthy lifestyles in order to prevent disease.

*********************************

\paragraph{Why we need NLP for family history extraction}

Modern health care system have enabled structured information about family history that are filled by patients through paper forms or on-line programs, however, a notable fraction of family history information is contained in free-text clinical notes, which are written by clinicians or xx after they encounter with patients.
\citet{polubriaginof-2015-amia-family-history} assessed the quality of family history data captured in an established commercial EHR at a medical centre. 
After analysing differences between 10,000 free-text and 9,121 structured family history observations, they find that free-text notes contain more information than the structured notes.


Most of these data are stored in unstructured/semi-structured format, therefore we need to employ NLP tools to convert these data into a structured format.
\begin{itemize}
    \item 
    \item 140,038 observations defined in the EHR; of those, 653 are family history related ~\cite{polubriaginof-2015-amia-family-history}.
\end{itemize}

% \footnote{\url{https://www.epic.com/}}
The Epic EHR includes a dedicated portion for collecting family history information.
The portion allows for structured entry of problems (selected from a list of 210 values such as cancer and diabetes), family member (selected from a list of 21 values such as mother and brother), age of onset (a numeric value such as 68), and a free-text field called \emph{comment}.
\citet{chen-vermont-2012-amia-family-history} conduct a manual review on $3,358$ unique comments to identify reasons for use of the comment field and what types of information are contained within them.
They find that greater than one-third of these comments are used to collect information that should be entered into available structured fields (a problem that can be selected from the list of 210 values or a specific onset age, such as `breast cancer at 70').






\section{Tasks and Resources}

In this section, we review what NLP tasks have been addressed in previous work, and what resources have been available to enable the development of NLP models for family history extraction.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/figure_tasks_studied.pdf}
    \caption{NLP Tasks studied in the literature.}
\end{figure}

\subsection{Tasks}

\paragraph{Family history sentence identification}

Although it is common to have a dedicated section of family history in clinical reports, \citet{lewis-ibm-2011-ieee-parsing-family-history} found that, in their dataset, only 36\% of family history information belongs to these dedicated sections. In other words, family history is buried in various places of clinical text, and usually mixed with patient medical history.
Therefore, the first component in a family history extraction pipeline is to determine if one sentence contains a family history statement~\citep{bill-minnesota-2014-amia-family-history}.

\paragraph{Family member detection}
The simplest format of family member detection task is to identify specific words, e.g., `brother', `son', in text that refer to the relative of the patient. However, there are several constraints that make the task less straightforward. The first one is that non-blood relatives, e.g., `adopted siblings', `partner's sister', are usually excluded as their information are not helpful to analyse familial history of the patient. The second one is that the possible surface forms need to be normalized with the side of family. For example, the family member described in `The mother has a brother who is an alcoholic and ...' is not the `brother' of the patient but the `uncle', and the side of family is `maternal'. The third issue is that information about two or more family members may be mentioned together. For example, there are two individuals mentioned in the sentence `both cousins suffered from high blood pressure', and the model needs to distinguish them when constructing the patient's family tree. %

\begin{itemize}
    \item Section segmentation: identifying a family history section and sentences within this section (IU)
    \begin{itemize}
        \item If clinical notes are CDA 1.0 compliant---sections have been codified, this step can skipped~\citep{mehrabi-mayo-2015-family-history}.
    \end{itemize}
    \item Entity identification, including family member and medical concept identification (IU; n2c2 2019). The family history elements may include disease, family member, cause, medication, age of onset of diagnosis, length of disease, etc~\citet{shen-mayo-2021-jmir-n2c2-2019-fh}.
    \item Living status
    \item Relation extraction, including relations between medical observations and family members  (IU; n2c2 2019)
    \item Negation detection  (IU; n2c2 2019).
\end{itemize}



\paragraph{Medical concept identification}
Depending on the downstream application, this may include any health-related problem including diseases, smoking, suicide and drinking~\cite{shen-mayo-2021-jmir-n2c2-2019-fh}.
Another challenge, pointed out by~\citet{shen-mayo-2021-jmir-n2c2-2019-fh}, is that medical observations beyond first or second degree should be excluded.

Diseases, diagnoses, various types of mutations, test results, treatments, and vital state.

\citet{lewis-sfsu-2011-bicob-family-history,lewis-ibm-2011-ieee-parsing-family-history} extract family history as a tuple consisting of a family member and a disease name, and the disease name must be resolvable to a 3 digit ICD9 code.

\paragraph{Clinical event recognition}
\citet{rama-oslo-2018-louhi-family-history} distinguish between clinical event (something happens and then is over, for example, the patient has a heart attachk) and clinical condition (a prolonged state, for example, the patient has heart disease).

\paragraph{Attributes}
Side; age; negation; amount; temporal

\paragraph{Relation}
hoder; moidifer; related to, subset

\paragraph{Other}
\citet{chen-vermont-2012-amia-family-history} focus on free-text comments within the `structured' family history section and aim to identify reasons for use of the comments field. 

\subsection{Resources}
Most of early studies on family history use in-house data, which are not publicly available. For example, \citet{friedlin-mcdonald-2006-amia-family-history} use admission notes dictated at a primary care hospital in Indianapolis, Indiana. \citet{goryachev-harvard-2008-amia-family-history} use discharge summaries and outpatient notes from two hospitals in Boston, Massachusetts. 
\citet{chen-vermont-2012-amia-family-history} use EHRs from a tertiary care academic medical center affiliated with the University of Vermont. 
Until recently, XXX.
We describe these openly available resources and provide a summary of these resources in Table~\ref{table-data-resource-summary}. %

MTSample dataset, used in~\citep{lewis-ibm-2011-ieee-parsing-family-history,lewis-sfsu-2011-bicob-family-history,bill-minnesota-2014-amia-family-history}, is an openly available resource that contains sample transcription reports for 40 specialties (e.g., general medicine, cardiovascular, urology). These reports have been anonymized and submitted by transcriptions and clinicians, and they can be used as a proxy of the kinds of texts generated in a clinical setting.
It is worthy noting that because MTSample is not a dedicated family history resource, the family history statements are relatively scarce.
\citet{lewis-ibm-2011-ieee-parsing-family-history} find that, out of 3940 clinical reports, there are only 1220 unique sentences mentioning at least one family member.
Similarly, \citet{bill-minnesota-2014-amia-family-history} find that only $284$ out of $23,155$ sentences contain family history statements.


To standardize evaluation on family history extraction, \citet{shen-mayo-2021-jmir-n2c2-2019-fh} organize the BioCreative/OHNLP family history extraction shared task in 2018 and then the n2c2/OHNLP shared task in 2019.
The 2019 shared task focuses on identifying family members and clinical observations, and extracting the association of the living status, side of the family and clinical observations with family members.
\citet{shen-mayo-2021-jmir-n2c2-2019-fh} curate the deidentified clinical narrative from family history sections of clinical notes at Mayo Clinic Rochester.
Note that automatically generated semi-structured texts and sections that combine the patients' social history with the family history are excluded in their corpus.
The corpus is annotated by a 5-member annotator team, and each document is annotated by 2 annotators.
One coordinator worked as the adjudicator to resolve discrepancies.

\citet{rama-oslo-2018-louhi-family-history} develop the annotation guidelines for family history extraction using synthetically produced clinical text in an iterative fashion. That is, the domain expert participates both in the annotation and development of guidelines. Synthetic examples are generated to challenge the annotation guidelines and then the guidelines are revised based on the annotation disagreements. %
In addition to `Family' members, \citeauthor{rama-oslo-2018-louhi-family-history} use `Self' to refer the patient under consideration, and `Index' to the proband---the first identified family member with a genetic disorder. Medical concepts---diseases, diagnoses, mutations, test results, treatments and vital state---are grouped into one entity category called `Condition'; `Event' (e.g., has a heart attack) is distinguished from `Condition' (e.g., have heart disease); a set of modifiers---side of the family, age, negation cues, amount, temporal---are annotated to assist semantic interpretation of family history information. \citeauthor{rama-oslo-2018-louhi-family-history} also define several relations between entities: holder (between Condition and Family/Self/Index entities); modifier (between modifiers and other entities); related to (between family members); subset (used when multiple family members are mentioned at the same time, e.g., between `two brothers' and `one of them'); partner (between no kinship family members that are able to provide offspring, e.g., between `husband' and `wife'). %

\citet{azab-umich-2019-emnlp-family-history} collect natural language interactions---answers to a family history questionnaire---and then annotate medical family histories. The questionnaire consists of questions targeting the medical history of the patient and their relatives up to third degree, and answers are collected from volunteers through crowd-sourcing or test cases of genetic counseling sessions. Finally, a genetic counseling expert manually annotate family members, their attributes (e.g., name, gender, age), and their illnesses. %
% If an illness is a cancer, a cancer type is also determined, choosing from a list of 23 types.

\begin{table}[t]
    \centering
    \begin{tabular}{c c p{0.35\linewidth}}
    \toprule
    Data & Size & Description \\
    \midrule
    n2c2/OHNLP 2019~\cite{shen-mayo-2021-jmir-n2c2-2019-fh} & 99 (Tr) 117 (Te) & \\
    UMich~\cite{azab-umich-2019-emnlp-family-history} & 4,304 sentences; 41,831 tokens & Cancer \\
    UiO~\cite{rama-oslo-2018-louhi-family-history} & 477 sentences; 6,030 tokens & Cardiac disease \\
    MTSamples~\citep{lewis-sfsu-2011-bicob-family-history} & 1274 reports & \multirow{3}{*}{Sample medical transcription reports} \\
    MTSamples~\citep{lewis-ibm-2011-ieee-parsing-family-history} & 3940 reports & \\
    MTSamples~\citep{bill-minnesota-2014-amia-family-history} & 491 reports & \\
    \bottomrule
    \end{tabular}
    \caption{A summary of openly available resources used in previous studies.}
    \label{table-data-resource-summary}
\end{table}

\iffalse
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm}p{8cm}c}
    \toprule
    Dataset & Description & Used in \\
    \midrule
    Indiana University (IU) & Clinical notes of patients who visited a hospital in Indianapolis during March-December 2013 & \citep{roch-2015-pancreatic-cyst,mehrabi-mayo-2015-family-history} \\
    \hline
    Mayo Clinic & Clinical notes for 2,923 patients with pancreatic cancer, extracted from the Mayo Clinic data repository & \citep{mehrabi-mayo-2015-family-history} \\
    \hline
    BioCreative/OHNLP 2018 & 99 patient notes from the Mayo Clinic Employee and Community Health. & \citep{dai-2019-bmc-family-member} \\
    \hline
    2019 n2c2/OHNLP track on family history extraction & & \citep{zhan-hit-2021-jmir-family-history} \\
    \hline
    Social History Annotation Corpus & & \citep{lybarger-washington-2021-jbi-sdoh} \\
    \bottomrule
    \end{tabular}
    \caption{A summary of available datasets.}
    \label{table-summary-datasets}
\end{table}
\fi

\section{Methods}

\subsection{Family history statement detection}
\begin{itemize}
    \item Rule-based
    \begin{itemize}
        \item SecTag~\citep{mehrabi-mayo-2015-family-history}
    \end{itemize}
\end{itemize}

\citet{lewis-sfsu-2011-bicob-family-history} identifies candidate family history sentences based on the presence of `sign-post' words (e.g., `mother', `brother'). They aim to extract family histories from any section within a clinical report, rather than only titled sections of family history~\citep{friedlin-mcdonald-2006-amia-family-history,goryachev-harvard-2008-amia-family-history}. %
\citet{bill-minnesota-2014-amia-family-history} use a classification approach of family history statement detection.
Their method takes the section heading, subsection heading and sentence text as input together, and then use N-gram-tokenized text as predictors to the SVM classifier.

\subsection{Relation extraction}
\citet{friedlin-mcdonald-2006-amia-family-history} develop a rule-based system for extracting family history for $12$ diseases and categorizing relative degrees (primary or secondary).
They first map noun phrases to the UMLS concepts of family member and diagnosis, and then use a set of co-occurrence based rules to associate diagnoses to family members.
When the system is evaluated on a set of $613$ hospital admission notes, it achieves greater than $.95$ sensitivity and positive predictive value for both disease extraction and relative categorization.

\begin{itemize}
    \item Ytex~\citep{mehrabi-mayo-2015-family-history}
    \item Deep-learning based~\citep{zhan-hit-2021-jmir-family-history}
\end{itemize}



\citet{almeida-matos-2020-sac-family-history} employ the Neji tool (\textcolor{red}{CITATION}), which relies on a dictionary complied from the UMLS Metathesaurus (\textcolor{red}{CITATION}).

 model entity identification as a sequence labeling problem using a CRF classifier, taking lexical features, part-of-speech features and manually designed binary features as input.


\citet{goryachev-harvard-2008-amia-family-history} employ a set of rules to associate the diagnosis with the most relevant family members.
Their method is able to accurately ($F_1$ score of $0.9231$) assign the diagnoses to specific family members, when evaluated on a set of $350$ sentences.
\citeauthor{goryachev-harvard-2008-amia-family-history} find that errors are likely to occur in those sentences with multiple groups of diagnoses or multiple groups of family members, whereas human annotators agree perfectly on these annotations.



\begin{itemize}
    \item Rule-based~\citep{mehrabi-mayo-2015-family-history}
    \item Deep-learning based~\citep{zhan-hit-2021-jmir-family-history}
\end{itemize}

\citet{almeida-matos-2020-sac-family-history} follow the shortest path in the dependency graph---build using Stanford CoreNLP (\textcolor{red}{CITATION})---to associate disease mentions to family members.





\paragraph{String matching}
\citet{bill-minnesota-2014-amia-family-history} rely on two external resources for family member detection and observation recognition.
That is, they search for matches to phrases in the HL7 Clinical Genomics family history model for family member detection and phrases defined by the UMLS Semantic Groups as disorders and procedures for observation recognition.
The identified family member and observation entities are then linked together by an indicator word or phrase thus forming a predication relation.
A lexicon of indicator words and phrases, including possession words (e.g., has, is, with) and experience indicators (e.g., suffered a, died of, recovered from), is constructed from the annotated training set.


\paragraph{Syntactic approach}
\citet{lewis-sfsu-2011-bicob-family-history} employs a set of dependency-based syntactic patterns to link a family member to its diagnosis. For example, if a sentence contains a direct object dependency (\emph{dobj}) and a nominal subject dependency (\emph{nsubj}), and both dependencies share the same governor, their method recognizes the dependent of the \emph{dobj} dependency as disease and the dependent of the \emph{nsubj} dependency as family member. %
% Their method achieves a precision of $0.79$ and recall of $0.58$ on the training set; and a precision of $0.61$ and recall of $0.51$ on the test set.
Similarly, \citet{lewis-ibm-2011-ieee-parsing-family-history} compile 107 unique dependency paths (e.g., `mother' $\to$ \emph{nsubj} $\to$ `has' $\to$ \emph{dobj} $\to$ `cancer') from 225 family history sentences.
They find that the most frequent 10 dependency paths can recover 57\% of the family history tuples.

\paragraph{Machine learning approach}
\citet{rama-oslo-2018-louhi-family-history} model entity (family member and observation) recognition as a sequence labeling problem using a linear SVM model.
The model takes features corresponding to individual word---lexical features of current and surrounding words, POS tags of current and surrounding words, and entity types of previous words---as input, and predict entity type for each word.
Similarly, \citet{azab-umich-2019-emnlp-family-history} use a CRF model for entity identification.  

For relation classification, a simil
\citet{rama-oslo-2018-louhi-family-history} uses a SVM model---based on lexical features, POS tags, dependency features, and entity types---for relation classification. 
\citet{azab-umich-2019-emnlp-family-history} builds a binary relation classifier to determine the relation between every pair of entities in the sentence.
The input features of the classifier include pre-trained word embeddings, position features and outputs from entity identification model, and a bi-directional LSTM classifier is used to determine whether the relation holds between given pair of entities.
\citeauthor{azab-umich-2019-emnlp-family-history} show that it can achieve high $F_1$ score---$0.98$---when a given sentence includes information regarding a single person, but relatively lower $F_1$---$0.87$---when the given sentence talks about two or more different persons.


\citet{zhan-hit-2021-jmir-family-history} propose a graph-based model with biaffine attention for family history extraction from cliniacl text.

\cite{azab-michigan-2019-emnlp-family-history} use a neural network with a CRF layer to produce attribute annotations, and then a neural network for binary classification of relations

\cite{bill-2014-amia-family-history} incorporate family history functionality into an open-source NLP system, BioMedICUS. It contains five pipeline components:

Family history sentence detection that determines if the sentence contains a family history statement.

Constituent mapping: annotate the family history members from the HL7 clinical genomics family history model as family-member entities, and annotate all the disorders or procedures from SNOMED CT as observation entities.

Relationship extraction: identified by “indicator phrases” (i.e., predication).
Coordination and list resolution: transforms relationships that have lists of family members and/or observations into a list of relationships that specify a single family member and single observation.

Attributes scanning: search patterns to identify the essential attributes of a relationship: vital status, certainty, age of diagnosis, side of family.




\subsection{Negation detection}
\begin{itemize}
    \item DEEPEN~\citep{mehrabi-mayo-2015-family-history}
    \item Rule-based~\citep{zhan-hit-2021-jmir-family-history}
\end{itemize}

The negation detection implementation in~\citep{bill-minnesota-2014-amia-family-history} scans terms to the left of the constituent object in question. 
Taking the phrase `father, but not mother' as an example, the negation component will add a negation attribute to only the `mother' entity of the phrase.


\section{Open Research Directions}

We identify challenges regarding data, task, modelling

\subsection{How can we obtain (annotated) data describing family history?}
The development of NLP models, especially models based on machine learning techniques, usually requires the access to manually annotated data.
Clinical text describing patients' family history

Synthetic data may not be fully representative of real clinical notes.

Health-related information stored in Electronic Health Records (EHRs) is private and should be protected.
Although some resources based on anonymized health records

governed by data

Common inter-annotator disagreement: semantic discrepancies (require domain knowledge) and temporal and negation-related information \cite{rama-2018-louhi-family-history}.

\citet{goryachev-harvard-2008-amia-family-history} find that the prevalence of family histories in clinical records is relatively low and family history information is not always documented clearly under sections `family history'.
In other

Previous studies rely on synthetic clinical text~\citep{rama-oslo-2018-louhi-family-history}

How do these models trained on synthetic clinical text perform on real world clinical text? How do they perform across different instituitions.

Cross text-type \citep{azab-umich-2019-emnlp-family-history}

\citet{azab-michigan-2019-emnlp-family-history} point out an interesting direction that a dialog agent may be able to collect data from the patient.

Clinical notes, admission reports, questionnaires

\subsection{How can we construct family tree from narrative texts?}
In addition to identifying 



\subsection{Clinician-AI interaction}
Hubert et al., (2022)

\citet{lewis-sfsu-2011-bicob-family-history} experiment with different visualization schemes---disease-centered view or family member centered view. However, it is unclear how clinicians interact with different views and how the interaction might affect clinician's perceptions toward system outputs.

\paragraph{Patient embeddings}

\paragraph{Can we infer the pedigree of a patient from text?}

text to pedigree chart? text to family graph? text to tabular formats directly usable in risk calcutators

\citet{rama-oslo-2018-louhi-family-history}: transform statemsnes about pedigree into tabular formats directly usable in risk calculators.

Given one patient's family history data, can we infer the pedigree chart, where nodes---the blood relatives of the patient---are organized in a tree structure.

Deploy a dialog agent to collect family history; away from pressured consultation environment 

\cite{Emery1999} point out that further work is needed to improve extraction of certainty and temporal modifications.

\cite{Friedlin2006,Welch2013,Lewis2011,goryachev-2008-amia-family-history}

Transferability: models trained on data from one institution may not work well on other institutions.


==> csur-archived/misc.tex <==

\noindent\fbox{%
    \parbox{\textwidth}{%
        \begin{itemize}
            \item The original plan was writing a survey of family history extraction. However, it is not easy to find a lot of related work on FHE. Citation numbers of these work are also very low. 
            \item We decide to focus on the topic of 'Patient-centric health risk identification'. 
            \begin{itemize}
                \item We focus on the idea of 'preventing', because if we cannot prevent healthy people from becoming patients, 'treating' causes larger impact on both people and health system 
                \item We emphasis `Patient-centric' here, because we want to identify health risks from patient-related data, such as EHR, in contrast to other sources such as scholarly articles
                \item We identify health risk from patient \emph{medical} history; \emph{family} history; and \emph{social} history. 
                \item Adverse drug events may be related as well, for example, we can identify risks from patient medical history, known allergies~\cite{mahendran-mcinnes-2021-amia-ade}. ADE caused by drug-drug interactions is excluded, because it is not 'patient-centric'
            \end{itemize}
        \end{itemize}
    }%
}

\paragraph{Why we need family history data}
Knowing that a patient is at increased risk of developing a disease based on family history enables disease prevention, varying from intensive screening to prophylactic surgery ~\cite{polubriaginof-2015-amia-family-history}.
For example, the risk assessment of hypertrophic cardiomyopathy considers 1 or more first-degree relatives with a history of sudden cardiac death under age 40 as a significant factor of sudden cardiac death risk \cite{shen-2021-jmir-n2c2-faimily-history}
The guidelines from the American Cancer Society recommend that patients who have a lifetime risk of breast cancer should have screening MRI in addition to mammography. The assessment heavily relies on family history and presence of risk factors ~\cite{polubriaginof-2015-amia-family-history}.

\cite{almeida-matos-2020-sac-family-history}
\cite{azab-umich-2019-emnlp-family-history}
\cite{bill-minnesota-2014-amia-family-history}
\cite{chen-vermont-2012-amia-family-history}
\cite{clift-mayo-2022-family-history}
\cite{dai-2019-bmc-family-member}
\cite{dai-csiro-2021-cikm-searchehr}
\cite{dai-nkust-2020-jmir-family-history}
\cite{endevelt-maccabi-2015-family-history}
\cite{friedlin-mcdonald-2006-amia-family-history}
\cite{goryachev-harvard-2008-amia-family-history}
\cite{lewis-ibm-2011-ieee-parsing-family-history}
\cite{lewis-sfsu-2011-bicob-family-history}
\cite{liu-mayo-2018-bio-creative}
\cite{lybarger-washington-2021-jbi-sdoh}
\cite{mehrabi-mayo-2015-family-history}
\cite{mehrabi-mayo-2016-amia-family-history}
\cite{milne-auckland-2009-family-hisory}
\cite{ozanne-drohan-2012-mri-screening}
\cite{permuth-egan-2009-familial-cancer}
\cite{polubriaginof-columbia-2015-amia-family-history}
\cite{rama-oslo-2018-louhi-family-history}
\cite{roch-2015-pancreatic-cyst}
\cite{rybinski-csiro-2021-jmir-family-history}
\cite{shen-mayo-2021-jmir-n2c2-2019-fh}
\cite{shi-hit-2019-bmc-family-history}
\cite{stubbs-kotfila-2015-jbi-i2b2-2014}
\cite{wang-mayo-2017-amia-family-history}
\cite{welch-kawamoto-2013-jamia-personalized-medicine}
\cite{zhan-hit-2021-jmir-family-history}

